2D-Guided 3D Gaussian Segmentation

Recently, 3D Gaussian, as an explicit 3D representation method, has demonstrated strong competitiveness over NeRF (Neural Radiance Fields) in terms of expressing complex scenes and training duration. These advantages signal a wide range of applications for 3D Gaussians in 3D understanding and editing. Meanwhile, the segmentation of 3D Gaussians is still in its infancy. The existing segmentation methods are not only cumbersome but also incapable of segmenting multiple objects simultaneously in a short amount of time. In response, this paper introduces a 3D Gaussian segmentation method implemented with 2D segmentation as supervision. This approach uses input 2D segmentation maps to guide the learning of the added 3D Gaussian semantic information, while nearest neighbor clustering and statistical filtering refine the segmentation results. Experiments show that our concise method can achieve comparable performances on mIOU and mAcc for multi-object segmentation as previous single-object segmentation methods.

==> Discussion.tex <==
\section{Limitation and Discussion}
% 由于本方法使用2D分割为指导，其不可避免地会受到2D分割结果的影响。如图所示，GT Mask中包含一部分的背景信息，所以他们出现在了分割结果中。此外，本方法还会受到场景重建质量的影响。在纹理特征不密集的区域，高斯会比较稀疏，距离其余同类别的高斯较远，因而会在统计滤波阶段被去除，这在图中也有所体现。对于因2D分割图的影响而将一些背景包含在3D高斯分割结果中的情况，一个可能的方法是在训练阶段加入深度信息，当3D高斯的深度突变时停止当前射线上的计算。
Since our method is guided by 2D segmentation maps, it is inevitably constrained by the outcomes of the 2D segmentation. As shown in Fig. \ref{Comparison}, the GT Mask includes some of the background information, so this also appears in the 3D Gaussian segmentation results. Additionally, our method is affected by the quality of the scene reconstruction. In regions where the texture features are not dense, the 3D Gaussian will be sparse and farther away from the rest of the 3D Gaussians of the same category, and thus will be removed in the statistical filtering stage, as depicted in Fig. \ref{Comparison}. For the case where some background is included in the 3D Gaussian segmentation result due to the influence of the 2D segmentation maps, a possible approach is to include depth information in the training phase and stop the computation on the current ray when the depth of the 3D Gaussian mutates.
